Verifiable Boosted Tree Ensembles

Verifiable learning advocates for training machine learning models amenable to efficient security verification. Prior research demonstrated that specific classes of decision tree ensembles -- called large-spread ensembles -- allow for robustness verification in polynomial time against any norm-based attacker. This study expands prior work on verifiable learning from basic ensemble methods (i.e., hard majority voting) to advanced boosted tree ensembles, such as those trained using XGBoost or LightGBM. Our formal results indicate that robustness verification is achievable in polynomial time when considering attackers based on the $L_\infty$-norm, but remains NP-hard for other norm-based attackers. Nevertheless, we present a pseudo-polynomial time algorithm to verify robustness against attackers based on the $L_p$-norm for any $p \in \mathbb{N} \cup \{0\}$, which in practice grants excellent performance. Our experimental evaluation shows that large-spread boosted ensembles are accurate enough for practical adoption, while being amenable to efficient security verification.

==> experiments-old.tex <==
\section{Experimental Evaluation}
\label{sec:experiments}
In this section we experimentally evaluate the key strengths and weaknesses of large-spread boosted ensembles. Our goal is understanding how much the large-spread restriction downgrades the performance of classifiers in non-adversarial settings and how much it improves their robustness in adversarial settings. Moreover, we evaluate the primary objective of our large-spread models, i.e., we assess whether they are amenable for efficient robustness verification.

\subsection{Methodology}
Our experimental evaluation is performed on three public datasets: Fashion-MNIST\footnote{\url{https://www.openml.org/search?type=data\&sort=runs\&id=40996&status=active}}, MNIST\footnote{\url{https://www.openml.org/search?type=data\&sort=runs\&id=554}} and Webspam\footnote{\url{https://www.csie.ntu.edu.tw/~cjlin/libsvmtools/datasets/binary.html}}. We reduce Fashion-MNIST and MNIST to binary classification tasks by considering two subsets of them. In particular, for Fashion-MNIST we consider the instances with class 0 (T-shirt/top) and 3 (Dress), while for MNIST we keep the instances representing the digits 2 and 6. The key characteristics of the chosen datasets are reported in Table~\ref{tab:datasets}. Each dataset is partitioned into a training set and a test set, using 70/30 stratified random sampling.

We then use the following methodology:
\begin{enumerate}
    \item We perform hyper-parameter tuning to identify the best-performing boosted tree ensemble trained using LightGBM. Evaluation is performed using traditional 3-fold cross-validation, looking for the ensemble with highest accuracy. We consider the following hyper-parameters: number of trees $m \in \{50,75,100,125,150\}$, maximal depth $D \in \{3,4,5,6,7\}$, number of nodes in $\{0.5*2^{(D+1)}-1, 0.75*2^{(D+1)}-1, 2^{(D+1)}-1\}$ and learning rate in $\{0.0001, 0.001, 0.01, 0.1\}$.
    \CLA{early stopping per alberi (max 500, patience=50 ). niente depth, num foglie 16, 32, 64, 128, 256.}
    
    \item We perform the same hyper-parameter tuning to identify the best-performing large-spread boosted tree ensemble trained using our algorithm. We do this for different norms ($L_\infty, L_0, L_1$) and different magnitudes of adversarial perturbations $k$.
    \item We assess the accuracy and robustness of both the traditional boosted ensemble and our large-spread ensemble to understand how the enforced model restriction impacts on classic performance measures in different settings (different norms and magnitudes of adversarial perturbations).
\end{enumerate}

There is an important point to stress here. Robustness verification for large-spread models can be efficiently performed using \tool, while traditional models without the large-spread restriction must be analyzed using existing verification tools. Since these tools may not scale on the entire test set, we enforce a timeout of 10 seconds per instance and we compute approximate values of robustness as required. In particular, when the verification tool goes in timeout, we consider its output as unknown, and we compute lower and upper bounds to robustness by considering such unknown instances as non-robust or robust respectively. We present approximate results using the $\pm$ notation. We finally assess the efficiency and scalability of robustness verification with respect to existing state-of-the-art tools in different settings.

\begin{table}[t]
\scalebox{0.87}{
    \centering
    \begin{tabular}{c|c|c|c}
    \toprule
    \textbf{Dataset} & \textbf{Instances} & \textbf{Features} & \textbf{Class Distribution} \\
    \midrule
    Fashion-MNIST & 13,866 & 784 & $50\% / 50\%$ \\
    MNIST & 14,000 & 784 & $51\% / 49\%$ \\
    Webspam & 350,000 & 254 & $70\% / 30\%$ \\
    \bottomrule
    \end{tabular}
}
\caption{Dataset statistics}
\label{tab:datasets}
\end{table}

\subsection{Case $p = \infty$}
We compare \tool{} against SILVA, a state-of-the-art verification tool for tree ensembles~\cite{RanzatoZ20}. SILVA uses abstract interpretation and in particular the hyper-rectangle abstract domain to perform exact robustness verification against attackers based on the $L_\infty$-norm.

\CLA{Alternative a "Traditional"? metterei LightGBM. oppure no-spread}
\LC{"no-spread" ci sta!}

\paragraph{Accuracy and Robustness Evaluation.}
Table~\ref{tab:measures_inf} compares the accuracy and the robustness of traditional models trained using LightGBM and our large-spread boosted ensembles. The first observation we make is that the large-spread restriction does not downgrade the accuracy of the trained models: in all cases, the accuracy of large-spread boosted ensembles is equivalent to the accuracy of traditional models. Although prior work already showed that large-spread ensembles can be accurate, some performance degradation was observed~\cite{CalzavaraCPP23}. Our use of boosting further weakens the practical limitations of the large-spread condition, likely because the trees of a boosted ensemble are specifically trained to compensate the weaknesses of their predecessors, yielding models which are equivalent to the state of the art. 

In turn, the large-spread condition is beneficial to robustness verification. Indeed, a state-of-the-art tool like SILVA can only provide approximate robustness bounds, because verification takes too much time. The bounds are rather large and make robustness verification unreliable: for many cases, the uncertainty is above $\pm 0.10$. For example, in the case of the Webspam dataset with $k = 0.0008$, robustness ranges between 0.61 and 0.97. This gap is unacceptable for a credible security verification. \tool{} is instead able to establish exact robustness bounds for our large-spread models. Observe that, in all cases, the robustness of large-spread models is close to the most optimistic robustness estimate obtained for the traditional models.

\begin{table}[t]
\scalebox{0.7}{
    \centering
    \begin{tabular}{c|c|c|c|c|c}
    \toprule
    \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{$k$}} & \multicolumn{2}{c}{\textbf{Accuracy}} & \multicolumn{2}{c}{\textbf{Robustness}} \\
    \cmidrule{3-6}
    & & Traditional & Large-Spread & Traditional & Large-Spread \\
    \midrule
    \multirow{3}{*}{FMNIST} & 0.0050 & \revise{0.97} & \revise{0.97} & \revise{0.93 $\pm$ 0.01} & \revise{0.96}\\
    & 0.0100 & \revise{0.97} & \revise{0.97} & \revise{0.81 $\pm$ 0.12} & \revise{0.89} \\
    & 0.0150 & \revise{0.97} & \revise{0.97} & \revise{0.68 $\pm$ 0.21} & \revise{0.88} \\
    \midrule
    \multirow{3}{*}{MNIST} & 0.0100 & \revise{0.99} & \revise{0.99} & \revise{0.98} & \revise{0.99} \\
    & 0.0200 & \revise{0.99} & \revise{0.99} & \revise{0.93 $\pm$ 0.02} & \revise{0.98} \\
    & 0.0300 & \revise{0.99} & \revise{0.99} & \revise{0.85 $\pm$ 0.10} & \revise{0.97} \\
    \midrule
    \multirow{3}{*}{Webspam} & 0.0004 & \revise{0.99} & \revise{0.99} & \revise{0.90 $\pm$ 0.08} & \revise{0.97} \\
    & 0.0006 & \revise{0.99} & \revise{0.99} & \revise{0.84 $\pm$ 0.13} & \revise{0.97} \\
    & 0.0008 & \revise{0.99} & \revise{0.99} & \revise{0.79 $\pm$ 0.18} & \revise{0.96} \\
    \bottomrule
    \end{tabular}
}
\caption{Accuracy and robustness measures for traditional and large-spread boosted ensembles. Robustness is computed against $A_{\infty,k}$ using SILVA on traditional boosted ensembles and \tool{} on large-spread boosted ensembles.
}
\label{tab:measures_inf}
\end{table}

\paragraph{Performance Evaluation.}
To better understand the performance of robustness verification, we carry out different experiments.

\begin{itemize}
    \item Fissare dimensioni lse migliore per ogni dataset, allenare equivalente tradizionale e raccogliere i tempi di verifica (tempo medio e deviazione standard) in tabella. Table~\ref{tab:time-inf}
    \item Fissare gli altri parametri e mostrare l'impatto del numero di alberi. Table~\ref{fig: scalability-inf}
    \item Fissare gli altri parametri e mostrare l'impatto della profondità. Figure~\ref{fig: scalability-inf}
\end{itemize} 


\begin{table}[t]
\scalebox{0.9}{
    \centering
    \begin{tabular}{c|c|c|c}
    \toprule
    \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{$k$}} & \multicolumn{2}{c}{\textbf{Verification Time}}\\
    \cmidrule{3-4}
    & & SILVA & CARVE-GBM\\
    \cmidrule{3-4}
    & & no-spread & lse \\
    \midrule
    \multirow{3}{*}{FMNIST} & 0.0050 & 101.078 & 54.983\\
    & 0.0100 & 6387.958 & 79.383 \\
    & 0.0150 & 18714.873 & 80.454 \\
    \midrule
    \multirow{3}{*}{MNIST} & 0.0100 & 1156.489 & 106.376 \\
    & 0.0200 & 3257.687 & 94.465 \\
    & 0.0300 & 8668.014 & 39.598 \\
    \midrule
    \multirow{3}{*}{Webspam} & 0.0002 & 5.421 &  31.258 \\
    & 0.0004 & 86.545 & 30.776 \\
    & 0.0006 & 296.003 & 15.989 \\
    & 0.0006 & 296.003 & 15.989 \\
    & 0.0006 & 296.003 & 15.989 \\
    \bottomrule
    \end{tabular}
}
\caption{Seconds}
\label{tab:time-inf}
\end{table}

\begin{figure*}[t]
  \centering
    \subfloat[\label{fig:time-efficiency}]{\includegraphics[width=.42\textwidth]{imgs/scalability_trees_inf_0.03.pdf}}
  \hfill
    \subfloat[\label{fig:memory-efficiency}]{\includegraphics[width=.42\textwidth]{imgs/scalability_depth_inf_0.03.pdf}}
  \caption{Comparison of the time required by SILVA and CARVE to verify the model on the entire MNIST test set.}
  \label{fig: scalability-inf}
\end{figure*}

\subsection{Case $p = 0$}

\paragraph{Accuracy and Robustness Evaluation.}

\begin{table}[t]
\scalebox{0.7}{
    \centering
    \begin{tabular}{c|c|c|c|c|c}
    \toprule
    \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{$k$}} & \multicolumn{2}{c}{\textbf{Accuracy}} & \multicolumn{2}{c}{\textbf{Robustness}} \\
    \cmidrule{3-6}
    & & Traditional & Large-Spread & Traditional & Large-Spread \\
    \midrule
    \multirow{3}{*}{FMNIST} & 1 & 0.97 & 0.96 & 0.93 & 0.95 \\
    & 3 & 0.97 & 0.96 & 0.86 & 0.92 \\
    & 5 & 0.97 & 0.96 & 0.72 & 0.87 \\
    \midrule
    \multirow{3}{*}{MNIST} & 1 & 0.99 & 0.99 & 0.98 $\pm$ 0.01 & 0.99 \\
    & 3 & 0.99 & 0.99 & 0.80 $\pm$ 0.01 & 0.98 \\
    & 5 & 0.99 & 0.99 & 0.42 $\pm$ 0.01 & 0.96 \\
    \midrule
    \multirow{4}{*}{Webspam} & 1 & 0.99 & 0.88 & 0.66 $\pm$ 0.19 & 0.75 \\
    & 2 & 0.99 & & & \\
    & 3 & 0.99 & 0.88 & 0.16 $\pm$ 0.16 & 0.40 \\
    & 5 & 0.99 & 0.88 & 0.17 $\pm$ 0.17 & 0 \\
    \bottomrule
    \end{tabular}
}
\caption{Accuracy and robustness measures for traditional and large-spread boosted ensembles. Robustness is computed against $A_{0,k}$ using Kantechelian on traditional boosted ensembles and CARVE on large-spread boosted ensembles.}
\label{tab:measures_0}
\end{table}

\paragraph{Performance Evaluation.}
\begin{itemize}
    \item Fissare dimensioni lse migliore per ogni dataset, allenare equivalente tradizionale e raccogliere i tempi di verifica (tempo medio e deviazione standard) in tabella. ~\ref{tab:time-0}
    \item Fissare gli altri parametri e mostrare l'impatto del numero di alberi.
    \item Fissare gli altri parametri e mostrare l'impatto della profondità.
\end{itemize}

\begin{table}[t]
\scalebox{0.9}{
    \centering
    \begin{tabular}{c|c|c|c|c}
    \toprule
    \multirow{3}{*}{\textbf{Dataset}} & \multirow{3}{*}{\textbf{$k$}} & \multicolumn{3}{c}{\textbf{Verification Time}}\\
    \cmidrule{3-5}
    & & \multicolumn{2}{c}{SILVA} & CARVE-GBM\\
    \cmidrule{3-5}
    & & no-spread & lse & lse \\
    \midrule
    \multirow{3}{*}{FMNIST} & 1 & 16.727 & 11.804 & 0.960 \\
    & 3 & 15.897 & 12.561 & 0.984 \\
    & 5 & 16.567 & 12.296 & 0.991 \\
    \midrule
    \multirow{3}{*}{MNIST} & 1 & 11.224 & 9.531 & 0.608\\
    & 3 & 11.228 & 9.345 & 0.603\\
    & 5 & 10.961 & 9.500 & 0.675\\
    \midrule
    \multirow{3}{*}{Webspam} & 1 & 14.415 & 5.539 & 0.077 \\
    & 2 &  &  & \\
    & 3 & 14.696 & 5.833 & 0.068\\
    & 5 & 14.455 & 5.811 & 0.077\\
    \bottomrule
    \end{tabular}
}
\caption{Seconds}
\label{tab:time-0}
\end{table}

\begin{figure*}[t]
  \centering
    \subfloat[\label{fig:time-efficiency}]{\includegraphics[width=.42\textwidth]{imgs/scalability_trees_0_5.pdf}}
  \hfill
    \subfloat[\label{fig:memory-efficiency}]{\includegraphics[width=.42\textwidth]{imgs/scalability_depth_0_5.pdf}}
  \caption{Comparison of the time required by \revise{SILVA} and CARVE to verify the model on the entire MNIST test set.}
  \label{fig: scalability-0}
\end{figure*}

\subsection{Case $p \in \N$}

\paragraph{Accuracy and Robustness Evaluation.}

\paragraph{Performance Evaluation.}
